On Designing Consistent Covariance Recovery from a Deep Learning Visual Odometry Engine

Deep learning techniques have significantly advanced in providing accurate visual odometry solutions by leveraging large datasets. However, generating uncertainty estimates for these methods remains a challenge. Traditional sensor fusion approaches in a Bayesian framework are well-established, but deep learning techniques with millions of parameters lack efficient methods for uncertainty estimation. This paper addresses the issue of uncertainty estimation for pre-trained deep-learning models in monocular visual odometry. We propose formulating a factor graph on an implicit layer of the deep learning network to recover relative covariance estimates, which allows us to determine the covariance of the Visual Odometry (VO) solution. We showcase the consistency of the deep learning engine's covariance approximation with an empirical analysis of the covariance model on the EUROC datasets to demonstrate the correctness of our formulation.

==> sections/methodology/incremental_covariance_recovery.tex <==
\subsection{Covariance recovery with a factor graph formulation in an incremental SLAM framework}
\begin{itemize}
    \item Matrix description of the information form in an incremental setting
    \item Effect of marginalization and state augmentation. 
    \item sliding window and covisibility graph
    \item Covariance update and propagation in an incremental setting.
\end{itemize}



